Deconstructing and reconstructing word embedding algorithms

Uncontextualized word embeddings are reliable feature representations of words used to obtain high quality results for various NLP applications. Given the historical success of word embeddings in NLP, we propose a retrospective on some of the most well-known word embedding algorithms. In this work, we deconstruct Word2vec, GloVe, and others, into a common form, unveiling some of the necessary and sufficient conditions required for making performant word embeddings. We find that each algorithm: (1) fits vector-covector dot products to approximate pointwise mutual information (PMI); and, (2) modulates the loss gradient to balance weak and strong signals. We demonstrate that these two algorithmic features are sufficient conditions to construct a novel word embedding algorithm, Hilbert-MLE. We find that its embeddings obtain equivalent or better performance against other algorithms across 17 intrinsic and extrinsic datasets.

==> covector.tex <==
\begin{table*}
\centering


\resizebox{\textwidth}{!}{%

\begin{tabular}{c|l|l}
\toprule
Probe $j$ 
& 
\multicolumn{1}{c|}{
$\argmax_i \hdot{i}{j}$
}
& 
\multicolumn{1}{c}{
$\argmax_i \hvec{i}\cdot \hvec{j}$ 
}
\\

\midrule

cat 
&
burglar, siamese, scan, scans, tabasco, schr\"odinger
& 
kittens, cats, kitten, poodle, terrier, dog 
\\

money
&
laundering, launder, extort, laundered, funneling
&
funds, monies, billions, cash, sums
\\


vector
&
tangent, scalar, subspace, dimensional, non-zero.
&
vectors, tensor, scalar, formula\_34, formula\_10
\\
\bottomrule

\end{tabular}
}
\caption{
High inner product, $\hdot{i}{j}$,  selects words that are compositionally compatible, whereas vector-vector dot products, $\hvec{i}\cdot\hvec{j}$, select words that can substitute one another.  ``Tabasco Cat'' is the name of a famous racehorse.
}
\label{table:covector}
\end{table*}

==> results/table_analogy.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{l rr}
    \toprule
        \textbf{Analogies} & Google & BATS\\
    \midrule
        SGNS     & \underline{.763} & .312  \\
        % SGNS-MF  & \textbf{.775} & \textbf{.354}  \\
        GloVe    & .739 & .310 \\
        % GloVe-MF & .745 & .324 \\
        \hilby   & .705 & \underline{.343}  \\
    \bottomrule
    \end{tabular}
    \caption{Results on analogy datasets using \textit{3CosMul}. Best is in \textbf{bold}.}
    \label{tab:analogy}
\end{table}

==> table-old.tex <==

\begin{table*}[t]
\centering
\begin{tabular}{c|l|c|c}
\textbf{Model} & 
\multicolumn{1}{c|}{$\hder$}
& \textbf{Objective} ($\phi_{ij}$)& \textbf{For}  

\rule{0pt}{0.8em}\rule[-0.8em]{0em}{0em}\\ \Xhline{3\arrayrulewidth}

%%%%%%%%%%%%% SGNS row %%%%%%%%%%%%% 
SGNS 
& 

\rule{0pt}{0em}
$(N_{ij} + N_{ij}^-) \cdot \Big[ 
\sigma \big(\hdot{i}{j}\big)
- \sigma\Big(\lg\frac{N_{ij}}{N_{ij}^-}\Big)
\Big]$

& 

$\pmi(i,j) - \ln k$

& 
$\forall (i,j)$

\rule{0pt}{1.5em}\rule[-1.1em]{0em}{0em}\\ \hline

%%%%%%%%%%%%% Glove row %%%%%%%%%%%%% 
GloVe

&

\rule{1.7em}{0em}
$2 h(N_{ij}) \cdot \Big[\hdot{i}{j} + b_i + b_j - \lg N_{ij} \Big]\quad\;$

&

$\approx \pmi(i,j)$

& 

$N_{ij}>0$

\rule{0pt}{1.5em}\rule[-1.0em]{0em}{0em}\\ \hline

%%%%%%%%%%%%% LDS row %%%%%%%%%%%%% 
LDS

& 

\rule{1.72em}{0em}
$4 h(N_{ij})
\cdot
\Big[
\norm{\hcovec{i}+\hvec{j}^\intercal}^2
-\lg N_{ij} + C
\Big]$

&

$d\cdot \pmi(i,j) - d\gamma$
& $N_{ij} > 0$

\rule{0pt}{1.5em}\rule[-1.0em]{0em}{0em}\\ \hline



%%%%%%%%%%%%% Swivel row %%%%%%%%%%%%% 
\multirow{2}{*}{Swivel\rule{0em}{1.8em}}
 
& 

\rule{2.52em}{0em}
$\sqrt{N_{ij}} \cdot \Big[ \hdot{i}{j} - \pmi(i,j) \Big]$

&

$\pmi(i,j)$

&

$N_{ij} > 0$

\rule{0pt}{1.5em}\rule[-1.0em]{0em}{0em}\\ 

& 

\rule{4.48em}{0em}
$1\cdot \sigma \Big(\hdot{i}{j} - \pmi^*(i,j) \Big)$

&

$\pmi^*(i,j)$

&

$N_{ij}=0$


\rule{0pt}{0em}\rule[-0.8em]{0em}{0em}\\ \Xhline{3\arrayrulewidth}


%%%%%%%%%%%%% Hilby row %%%%%%%%%%%%% 
\hilby

& 

\rule{1.69em}{0em}
$\big(p_i p_j\big)^\frac{1}{\tau} \cdot \Big[
e^{\hdot{i}{j}}
- e^{\pmi(i,j)}
\Big]$

&

$\pmi(i,j)$

&

$\forall (i,j)$
\rule{0pt}{2.5em}\rule[-0em]{0em}{0em}\\ 

    \end{tabular}
    \caption{Comparison of low rank embedders.  
    $h(N_{ij})$ is defined in Eq.4.
    See original works for  new symbols: SGNS \cite{mikolov2013distributed}, GloVe \cite{pennington2014glove}, LDS \cite{arora2016latent}, Swivel \cite{shazeer2016swivel}.
    }
    \label{tab:embedder-form-comparison}
\end{table*}
